Attacker Control and Impact for Confidentiality and Integrity

Language-based information flow methods offer a principled way to enforce strong security properties, but enforcing noninterference is too inflexible for realistic applications. Security-typed languages have therefore introduced declassification mechanisms for relaxing confidentiality policies, and endorsement mechanisms for relaxing integrity policies. However, a continuing challenge has been to define what security is guaranteed when such mechanisms are used. This paper presents a new semantic framework for expressing security policies for declassification and endorsement in a language-based setting. The key insight is that security can be characterized in terms of the influence that declassification and endorsement allow to the attacker. The new framework introduces two notions of security to describe the influence of the attacker. Attacker control defines what the attacker is able to learn from observable effects of this code; attacker impact captures the attacker's influence on trusted locations. This approach yields novel security conditions for checked endorsements and robust integrity. The framework is flexible enough to recover and to improve on the previously introduced notions of robustness and qualified robustness. Further, the new security conditions can be soundly enforced by a security type system. The applicability and enforcement of the new policies is illustrated through various examples, including data sanitization and authentication.

==> abstract.tex <==
Language-based information flow methods offer a principled way to
enforce strong security properties, but enforcing noninterference
is too inflexible for
realistic applications. Security-typed languages have therefore
introduced declassification mechanisms for relaxing confidentiality
policies, and endorsement mechanisms for relaxing integrity policies.
However, a continuing challenge has been to define what security is
guaranteed when such mechanisms are used.
%
This paper presents a new semantic framework for expressing security
policies for declassification and endorsement in a language-based
setting. The key insight is that security can be described in terms of
the power that declassification and endorsement give the attacker. The
new framework specifies how attacker-controlled code affects program
execution and what the attacker is able to learn from observable
effects of this code.
%
This approach yields novel security conditions for checked
endorsements and robust integrity. The framework is flexible enough to
recover and to improve on the previously introduced notions of
robustness and qualified robustness.  Further, the new security
conditions can be soundly enforced by a security type system. The
applicability and enforcement of the new policies is illustrated
through various examples, including data sanitization and
authentication.

